Structural Agnostic Modeling: Adversarial Learning of Causal Graphs

A new causal discovery method, Structural Agnostic Modeling (SAM), is presented in this paper. Leveraging both conditional independencies and distributional asymmetries, SAM aims to find the underlying causal structure from observational data. The approach is based on a game between different players estimating each variable distribution conditionally to the others as a neural net, and an adversary aimed at discriminating the generated data against the original data. A learning criterion combining distribution estimation, sparsity and acyclicity constraints is used to enforce the optimization of the graph structure and parameters through stochastic gradient descent. SAM is extensively experimentally validated on synthetic and real data.

==> SAM_section_0.tex <==
\begin{abstract}
A new causal discovery method, {\em Structural Agnostic Modeling} (SAM), is presented in this paper. Leveraging both conditional independencies and distributional asymmetries, SAM aims to find the underlying causal structure from observational data. 
The approach is based on a game between different players estimating each variable distribution conditionally to the others as a neural net, and an adversary aimed at discriminating the generated data against the original data. A learning criterion combining distribution estimation, sparsity and acyclicity constraints is used to enforce the  optimization of the graph structure and parameters through stochastic gradient descent. SAM is extensively experimentally validated on synthetic and real data.
\end{abstract}

==> SAM_section_1.tex <==
\section{Introduction}
This paper addresses the problem of uncovering causal structure from multivariate observational data. This problem is receiving more and more attention with 
the increasing emphasis on model interpretability and fairness  \citep{Velez17}.
%and robust learned models gives causal modeling a renewed importance. %
While the gold standard to establish causal relationships remains randomized controlled experiments \citep{Pearl03,Imbens_book}, in practice these often happen to be costly, unethical, or simply infeasible.
%
Therefore, hypothesizing causal relations from observational data, often referred to as {\em observational causal discovery}, has attracted much attention from the machine learning community \citep{lopez2015towards,mooij2016distinguishing,PetJanSch17}.
%
Observational causal discovery has found many applications, e.g. in economics to understand and model the impact of monetary policies \citep{chen2007causal}, or in bio-informatics to infer network structures from gene expression data \citep{sachs2005causal} and prioritize  exploratory experiments.


% The Functional Causal Model (FCM) framework \citep{pearl2003causality} formalizes the causal structure of $d$ variables $\mathbf{X} = (X_1, \ldots, X_d)$ through a set of equations (more in Section \ref{sec:problem_setting}):
% \begin{equation}
%     X_i = f_i(X_{\text{Pa}(i)}, E_i), 
%   \label{eq:fcm}
% \end{equation}
% for $i = 1, \ldots, d$, where $\text{Pa}(i)$ denotes the set of the direct causes of $X_i$, $E_i$ is a random noise accounting for other unobserved causes for $X_i$, and $f_i$, referred to as {\em causal mechanism}, is a deterministic function determining the value of effect variable $X_i$ from the values of causes $X_{\text{Pa}{(i)}}$ and noise $E_i$. Formally, an FCM is characterized as a causal graph $\mathcal{G}$, involving all variables as nodes, where each directed (respectively undirected) edge $X_i-X_j$ stands for a direct causal relation from $X_j$ to $X_i$ (resp. a dependency between $X_i$ and $X_j)$.

Observational causal discovery aims to learn  the causal graph from samples of the joint probability distribution of observational data. Four
%\NOTE{4 et pas 3, modifé par conformité avec section3.}
main approaches have been proposed in the literature (more in Section \ref{sec:soa}).

A first approach refers to score based methods, using local search operators to navigate in the space of Directed Acyclic Graphs (DAGs) in order to find the Markov equivalence class of the graph
%, corresponding to the lowest score
optimizing the considered score
\citep{chickering2002optimal,ramsey2015scaling}. A second approach
%represent 
includes
constraint-based methods leveraging conditional independence tests to identify the skeleton of the graph and the v-structures \citep{spirtes1993search,colombo2012learning}. A third approach embodies hybrid algorithms, combining ideas from constraint-based and score-based algorithms \citep{tsamardinos2006max,ogarrio2016hybrid}. 
The fourth approach goes beyond the Markov equivalence class limitations by exploiting asymmetries in the joint distribution,
%. For example in the bivariate case, it is based on
e.g. based on 
the assumption that $p(x)p(y|x)$ is simpler than $p(y)p(x|y)$ (for some appropriate notion of simplicity) when $X$ causes $Y$ 
%($X \rightarrow Y$) 
\citep{hoyer2009nonlinear,zhang2010distinguishing,stegle2010probabilistic}.  Another stream of work closely related to causal discovery is the {\em causal feature selection}, aiming at recovering the Markov Blanket of %given 
target variables \citep{yu2018unified}. It leverages the estimation of mutual information among variables \citep{bell2000formalism,brown2012conditional,vergara2014review} or 
%leveraging 
uses classification or regression models 
%by performing 
to support variable selection  \citep{aliferis2003hiton,aliferis2010local}.



The contribution of this paper is a new causal discovery algorithm called {\em Structural Agnostic Modeling} (SAM),\footnote{Available at \url{https://github.com/Diviyan-Kalainathan/SAM}.} restricted to continuous variables, which aims to exploit both conditional independence relations and distributional asymmetries from observational data. 
SAM searches for an acyclic Functional Causal Model (FCM) \citep{Pearl03}.

SAM proceeds as follows: i) the distribution of each variable conditionally to its parents, referred to as Markov kernel \citep{janzing2010causal}, is learned from the observational data as a neural net;  ii) sparsity and acyclicity constraints are defined on the graph derived from these Markov kernels, inspired from \cite{leray1999feature,yu2018unified,Dag-no-tears}; iii) all Markov kernels are learned in parallel, subject to the above constraints, through an adversarial mechanism, discriminating the true data distribution from the partial distributions generated after the Markov kernels  \citep{goodfellow2014generative,mirza2014conditional}. The critical combinatorial optimization problem at the core of (causal) graph learning thus is tackled through a single continuous optimization problem. 

Overall, SAM relies on Occam's razor principle to infer the causal graph,
using compound structural and  functional complexity scores to assess the complexity of each candidate graph.

This paper is organized as follows:  Section \ref{sec:problem_setting} introduces the problem of learning an FCM, presents the main underlying assumptions and briefly describes the state of the art in causal modelling. Section \ref{sec:problem} presents the principle of the proposed approach and its loss function. Section \ref{sec:practical} describes the SAM algorithm devised to optimize this loss function. Section \ref{sec:first_exp} presents the experimental setting used for the empirical validation of SAM and provides illustrative examples on causal graph learning. Section \ref{sec:benchmarks} reports on SAM empirical results compared to the state of the art.  Section \ref{sec:conclusion} discusses the contribution and presents some perspectives for future work.


==> SAM_section_2.tex <==
\def\X{\mbox{$\mathbf{X}$}}
\def\x{{\mathbf{x}}}
\newcommand{\NOTE}[1]{{\footnote{\bf #1 (ms)}}}

\section{Observational Causal modeling: Formal Background} \label{sec:problem_setting}

Let $\mathbf{X} = \left[X_1,\ldots X_d\right]$ denote a 
vector of $d$ continuous random variables, with unknown joint probability distribution $p(\mathbf{X})$ and joint density $p(\x)$. The observational causal discovery setting considers $n$ iid samples drawn from $p(\mathbf{X})$, noted $D = \{\x^{(1)},\ldots, \x^{(n)}\}$, with $\x^{(\ell)} = (x^{(\ell)}_1, \ldots, x^{(\ell)}_d)$ and $x^{(\ell)}_j$ the $\ell$-th sample of $X_j$. 

\subsection{Functional Causal Models \label{sec:FCM}} 
The underlying generative model of the data is assumed to be a Functional Causal Model (FCM) \citep{Pearl03}, defined as a pair $(\mathcal{G}, f)$, with $\mathcal{G}$ a directed acyclic graph and $f = (f_1,\ldots, f_d)$ a set of $d$ causal mechanisms. Formally, we assume that each variable $X_j$ follows a distribution described as: 
\begin{equation}  
{X}_j = f_j({X}_{\Pa{j}}, {E}_j).
    \label{eq:fcm}
\end{equation}


For notational simplicity, $X_j$ denotes both a variable and the associated node in graph $\mathcal{G}$. $\Pa{j}$ is the set of parents of $X_j$ in $\mathcal{G}$, $f_j$ is a function from $\mathbb{R}^{|\Pa{j}|+1} \rightarrow \mathbb{R}$ and ${E}_j$ is a random noise variable modelling the effects of non-observed variables.
%\footnote{Note that this is not an actual restriction on the FCM space, as any type of noise can be modeled as some $g(E)$ with $g$ a function and $E$ a Gaussian noise  \citep{stegle2010probabilistic}.}, accounting for all unobserved causes of $X_j$.

A 5-variable FCM is depicted on Figure \ref{figure:causalnetwork}.

\begin{figure}[h]
    \centering
    \begin{tikzpicture}[node distance=0.25cm, auto,]
        \node[punkt, dotted] (e2) at (0,0) {$E_1$};
        \node[below=of e2] (f2) {$f_1$};
        \node[punkt, below=of f2] (x2) {$X_1$};
        \node[punkt, dotted, right=1cm of x2] (e4) {$E_3$};
        \node[punkt, dotted, left=1cm of x2] (e3) {$E_2$};
        \node[punkt, dotted, right=2cm of e4] (e5) {$E_4$};
        \node[below=of e5] (f5) {$f_4$};
        \node[punkt, below=of f5] (x5) {$X_4$};
        \node[punkt, dotted, left=1cm of x5] (e6) {$E_5$};
        \node[below=of x2, shift={(-0.8cm,0)}] (f3) {$f_2$};
        \node[right=1cm of f3] (f4) {$f_3$};
        \node[punkt, below=of f4] (x4) {$X_3$};
        \node[below=of e6] (f6) {$f_5$};
        \node[punkt, below=of f6] (x6) {$X_5$};
        \node[punkt, below=of f3] (x3) {$X_2$};

        \draw[pil] (e2) -- (f2);
        \draw[pil] (e3) -- (f3);
        \draw[pil] (e4) -- (f4);
        \draw[pil] (e5) -- (f5);
        \draw[pil] (e6) -- (f6);

        \draw[pil] (f2) -- (x2);
        \draw[pil] (f3) -- (x3);
        \draw[pil] (f4) -- (x4);
        \draw[pil] (f5) -- (x5);
        \draw[pil] (f6) -- (x6);

        \draw[pil] (x2) -- (f3);
        \draw[pil] (x2) -- (f4);
        \draw[pil] (x4) -- (f6);
        \draw[pil] (x5) -- (f6);

        \node[right=1.75cm of f5] {
                $\begin{cases}
                X_1 = f_1(E_1) \\
                X_2 = f_2(X_1,E_2) \\
                X_3 = f_3(X_1,E_3) \\
                X_4 = f_4(E_4) \\
                X_5 = f_5(X_3,X_4,E_5) \\
                \end{cases}$};
    \end{tikzpicture}
    \caption{Example of a Functional Causal Model (FCM) on $\mathbf{X} = [X_1, \ldots, X_5]$. Left: causal graph $\mathcal{G}$. Right: causal mechanisms.}
    \label{figure:causalnetwork}
\end{figure}


\subsection{Notations and Definitions}

%\NOTE{Je rajoute $D$  et $S$ ds la table.\\ Is $p(x)$ the true or the empirical distribution ? $p(x)$ is the true distribution (Olivier)}
%ok.
All notations used in the paper are listed in Appendix \ref{sec:notations}.
%on l'a dit moins d'une demi page plus haut, je l'enlève
%We briefly remind that $X_j$ denotes a variable and its associated node in graph $\mathcal{G}$.
$\textbf{X}_{\backslash i}$ denotes the set of all variables but $X_i$. \\
\textbf{\em Conditional independence}: $(X_i \indep X_j|X_k)$ means that variables $X_i$ and $X_j$ are independent conditionally to $X_k$, i.e. $p(x_i,x_j|x_k) = p(x_i|x_k)p(x_j|x_k)$.\\
\textbf{\em Markov blanket}: a Markov blanket $\text{MB}(X_i)$ of a variable $X_i$ is a minimal subset of variables in $\textbf{X}_{\backslash i}$ such that any disjoint set of variables in the network is  independent of $X_i$ conditioned on $\text{MB}(X_i)$.\\
\textbf{\em V-structure}: Variables $\{X_i, X_j, X_k\}$ form a v-structure iff their causal structure, in the induced subgraph of $\mathcal{G}$ with these three variables, is : $X_i \rightarrow X_k \leftarrow X_j$.\\
\textbf{\em Skeleton of the DAG}: the skeleton of the DAG  is the undirected graph obtained by replacing all edges by undirected edges.\\
\textbf{\em Markov equivalent DAG}: two DAGs with same skeleton and same v-structures  are said to be \textit{Markov equivalent} \citep{pearl1991formal}. A \textit{Markov equivalence class} is represented by a \textit{Completed Partially Directed Acyclic Graph} (CPDAG) having both directed and undirected edges.

Variables $X_i$ and $X_j$ are said to be adjacent according to a CPDAG iff there exists an edge between both nodes. If directed, this edge models causal relationship $ X_i \rightarrow X_j$ or $X_j  \rightarrow X_i$. If undirected, it models a causal relationship in either direction.





\subsection{Causal Assumptions and Properties \label{sec:assumption}} 
In this paper, we make the following assumptions: 

\paragraph{Acyclicity:}
The causal graph $\mathcal{G}$ (Equation  (\ref{eq:fcm})) is assumed to be a Directed Acyclic Graph (DAG). 


\paragraph{Causal Markov Assumption (CMA):}
Noise variables $E_j$ (Equation (\ref{eq:fcm})) are assumed to be independent from each other. This assumption together with the above DAG assumption yields the classical causal Markov property, stating that all variables are independent of their non-effects (non descendants in the causal graph) conditionally to their  direct causes (parents) \citep{spirtes2000causation}. Under the causal Markov assumption, the distribution described by the FCM satisfies all conditional independence relations\footnote{It must be noted however that the data might satisfy additional independence relations beyond those in the graph; see the faithfulness assumption.} among variables in $\mathbf{X}$ via the notion of d-separation \citep{pearl2009causality}.  Accordingly the joint density $p(\x)$ can be factorized as the product of the densities of each variable conditionally on its parents in the graph:

\begin{equation}  
p(\x) = \prod_{j=1}^{d} p(x_j | x_{\Pa{j}})
\end{equation}


\paragraph{Causal Faithfulness Assumption (CFA):}

The joint density $p(\x)$ is assumed to be \textit{faithful} to graph $\mathcal{G}$, that is, every conditional independence relation that holds true according to  $p$ is entailed by $\mathcal{G}$ \citep{spirtes2016causal}. 
It follows from causal Markov and faithfulness assumptions that every causal path in the graph corresponds to a dependency between variables, and vice versa.

\paragraph{Causal Sufficiency assumption (CSA):}  

$\mathbf{X}$ is assumed to be \textit{causally sufficient}, that is, a pair of variables $\{X_i, X_j\}$ in $\mathbf{X}$ has no common cause external to $\textbf{X}_{\backslash i,j}$. In other words, we assume that there is no hidden confounder. 
This corresponds to making the assumption that the noise variables $E_j$ for $j=1,..,d$ entering in Equation (\ref{eq:fcm}) are independent of each other. 




% Accordingly, any candidate model can be viewed as a Bayesian network representing a joint distribution. This formalization can  be used to characterize and simulate the distribution resulting from an intervention (setting some variable $X_j$ to some constant $v_j$), referred to as \emph{interventional distribution} and noted $q_{\text{do}(X_j = v_j)}(x)$ \citep{pearl2009causality}. Formally, such an interventional 
% distribution is computed from the candidate model by discarding all causal influences on $X_j$ and clamping its value to $v_j$.\\
% \isabelle{La phrase du dessus est candidate a la suppression. Ca va plutot dans l'introduction.}
% Contrasting with Bayesian networks, 
% \isabelle{Juste avant il est dit qu'un FCM est un BN, clarifier}
% the FCM framework may support counterfactual analysis on individual samples $-$ while Bayesian networks only support the evaluation of intervention impacts at the distribution level \citep{pearl2009causality}. Practically, for any $d$-dimensional sample $\x^{(\ell)} = (x^{(\ell)}_1, \ldots, x^{(\ell)}_d)$ and for $j$ in $1 \ldots d$, if the function $f_j$ is injective, one can infer the  value $e^{(\ell)}_j$ of noise variables $E_j$  such that: $$x^{(\ell)}_j = \hat{f}_j(x^{(\ell)}_{\Pahat{j}},e^{(\ell)}_j).$$
% When facing any intervention $X_j = v_j$ and accordingly setting $x^{(\ell)}_j = v_j$, the inferred $e^{(\ell)}_j$ are used to recompute every $x^{(\ell)}_k$ (likewise with $k$ ordered in the topological order of $\widehat{\mathcal{G}}$), thus answering the question of "how would sample $\x^{(\ell)}$ be modified under interventions". 

% \michele{Mais on n'a dit nulle part que fj est injective... J'ai manqué une étape ici, discutons-en.} 
% \olivier{Heu oui, bonne remarque, j'ai ajouté cette hypothèse dans ce cas.  }

% \isabelle{A mon avis, tu en dis trop ou pas assez sur les counterfactuals. Et un petit croquis ferait mieux qu'un long discours... Est-ce important? Je croyais que le papier n'etait pas sur l'inferrence mais sur le causal discovery. Je ne vois pas clairement ce qui est utile dans la section 2.5 pour le reste du papier (surtout les experiences).}

% \isabelle{The introduction presents the problem as that of uncovering the causal graph. But here the model reproduces the values of the variables, not just the graph structure. The goal of the paper should be clarified.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STATE OF THE ART %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Background \label{sec:soa}}

%\isabelle{This section needs to be put in the light of the goal(s) of the paper. Each algorithm family should come with advantages and limitations, so it will become clear that fusing ideas will give you the best of all worlds.}

%\olivier{Ok c'est fait, on a grandement réduit cette section. On renvoit le lecteur aux annexes pour plus de détails. Après on verra si les annexes sont trop longues on pourra en enlever. Mais bon c'est peut être pas mal pour un article de journal d'avoir un état de l'art un peu conséquent dans un coin quand même non ? }




This section briefly presents a formal background of observational causal discovery, referring the reader to \citep{spirtes2000causation,PetJanSch17}  for a comprehensive survey. 
%\michele{Je pense qu'il faut situer ici LiNGAM - Hyvarinen (surtout qu'on l'a comme basline). Son approche était dominante à Oberwolfach.}
%\olivier{Oui ok c'est vrai qu'on l'avait un peu oublié dans le SoA. Je l'ai ajouté en début de III. C'est curieux qu'ils disent que ça soit une approche dominante. La méthode marche super mal en pratique  sur des données réalistes}

Observational causal discovery algorithms are structured along four categories:



\begin{enumerate}
    \item[I] A first category of methods are score-based methods which aim to find the best CPDAG in the sense of some global score:  using search heuristics, graph candidates are iteratively evaluated using a scoring criterion such as the AIC score or the BIC score and compared with the best graph obtained so far. One of the most popular score-based method is the Greedy Equivalent Search (GES) algorithm \citep{chickering2002optimal}. GES  aims to find the best CPDAG in the sense of the Bayesian Information Criterion (BIC). The CPDAG space is navigated using local search operators, e.g. \textit{add edge}, \textit{remove edge}, and \textit{reverse edge}. GES starts with an empty graph. In a first forward phase, edges are iteratively added to greedily improve the global score.  In a second backward phase, edges are iteratively removed to greedily improve the score. Under CSA, CMA and CFA assumptions, GES identifies the true CPDAG in the large sample limit, if the score used is decomposable, score-equivalent and consistent \citep{chickering2002optimal}. More recently, \cite{ramsey2017million} proposed a GES extension called Fast Greedy Equivalence Search (FGES) algorithm aimed to alleviate the computational cost of GES. It leverages the decomposable structure of the graph to optimize all the subgraphs in parallel. This optimization greatly increases the computational efficiency of the algorithms, enabling score-based methods to run on millions of variables.

   \item[II] A second category of approaches are constraint-based methods leveraging conditional independence tests to identify a skeleton of the graph and v-structures, in order to output the CPDAG of the graph. 
One of the most famous constraint-based algorithm is the celebrated PC algorithm \citep{spirtes1993search}: under CSA, CMA and CFA, and assuming  that all conditional independences have been identified, PC returns the CPDAG of the functional causal model, respecting all v-structures.  It has notably been shown that  for  graphs  with  bounded  degree, the PC algorithm has a running time that is polynomial in the number of variables. When very fast independence tests such as partial correlation tests are employed, the PC algorithm can handle high dimensional graphs \citep{kalisch2007estimating}. 
For non Gaussian data generated with non-linear mechanisms and complex interactions between the variables, more powerful but also more time consuming  tests  have been proposed such has the Kernel  Conditional  Independence  test  (KCI) \citep{zhang2012kernel} leveraging the kernel-based Hilbert-Schmidt Independence Criterion (HSIC) \citep{gretton2005kernel}.

\item [III] The third category of approaches are hybrid algorithms which combine ideas from constraint-based and score-based algorithms. According to \cite{nandy2015high}, such methods often use a greedy search like the GES method on a restricted search space for the sake of computational efficiency. This restricted space is defined using conditional independence tests. The Max-Min Hill climbing algorithm (MMHC) \citep{tsamardinos2006max} firstly builds the skeleton of a Bayesian network using conditional independence tests (using constraint-based approaches) and then performs a Bayesian-scoring hill-climbing search to orient the edges (using score-based approaches). The skeleton recovery phase, called Max-Min Parents and Children (MMPC) selects for each variable its parents and children in the 
%dataset. 
variable set. Note that this task is different from recovering the Markov blanket of variables as the spouses are not selected. The orientation phase is a hill-climbing greedy search involving 3 operators: {\em add, delete} and {\em reverse edge}.


%The fourth category are structural equation models with parametric assumptions. 

\item [IV]   The 
% three 
above-mentioned 
three categories of methods can learn at best the Markov equivalence class of the DAG  which can be a significant limitation in some cases\footnote{In the case where the  sought $\cal G$ graph does not include v-structures (e.g., due to its being star-shaped),  the cited methods are unable to orient the edges (see section \ref{subsec:biologic_syntren}).}. Therefore, new methods exploiting asymmetries or causal footprints in the data generative process have been proposed to uniquely identify the causal DAG. According to \cite{quinn2011learning}, the first approach in this direction is LiNGAM  \citep{shimizu2006linear}. LiNGAM handles linear structural equation models on continuous variables, where each variable is modeled as the weighted sum of its parents and noise. Assuming further that all noise variables are non-Gaussian, \cite{shimizu2006linear} show that the causal structure is fully identifiable (all edges can be oriented). 

Such methods, taking into account the full information from the observational data \citep{spirtes2016causal} such as data asymmetries induced by the causal directions, have been proposed and primarily applied to the bivariate DAG case\footnote{Note that in the bivariate case, both $X \rightarrow Y$ and $Y \rightarrow X$ DAGs are Markov equivalent; methods in categories I, II and III
do not apply.}, referred to as cause-effect pair problem
\citep{hoyer2009nonlinear,daniusis2012inferring,mooij2016distinguishing, zhang2010distinguishing}. The reader is referred to \cite{statnikov2012new,mooij2016distinguishing, guyon2019cause} for a thorough presentation of the bivariate problem. 
The extension of the bivariate approaches to the multivariate setting has been tackled by \cite{Friedman2000,buhlmann2014cam} assuming additive noise, and identifiability results have been obtained for the causal additive models (CAM) \citep{buhlmann2014cam}. 

As noted by \cite{stegle2010probabilistic}, identifiability results (see e.g. \citep{hoyer2009nonlinear,zhang2010distinguishing,buhlmann2014cam} most often rely on restrictions on the class of admissible causal mechanisms; however, such restrictions might be too strong for real-world data.

In order to overcome such a limitation and build more expressive models,  \cite{stegle2010probabilistic} have  proposed the fully  non-parametric   GPI approach.  The key idea is to define appropriate priors on marginal distributions of the causes and on causal mechanisms in order to favor a model of low complexity. This method, designed for the bivariate setting, has shown very good results on a wide variety of data as it is not restricted to a specific class of mechanisms. 

Extending this complexity-based search to the multivariate case, the Causal Generative Neural Networks (CGNN) \citep{goudet2018learning} uses generative neural networks to model the causal mechanisms. CGNN starts from a given skeleton and explores the space of DAGs using a hill climbing algorithm aimed to optimize  the global score of the network computed as the Maximum Mean Discrepancy  (MMD) \citep{gretton2007kernel} between the true empirical distribution $P$ and the generated distribution $\widehat{P}$. 
\end{enumerate}


The proposed SAM approach ambitions to combine the best of all the above: exploiting conditional independence relations as methods in the first three categories, and exploiting distributional asymmetries, achieving some trade-off between model complexity and data fitting in the line of the GPI method \citep{stegle2010probabilistic}. 
    
SAM aims at addressing the limitations of CGNN.  The first limitation of CGNN is a quadratic computational complexity w.r.t. the size of the dataset, as its learning criterion is based on the Maximum Mean Discrepancy between the generated and the observed data. 
In contrast, SAM uses an adversarial learning approach (GAN) \citep{goodfellow2014generative} that scales linearly with the data size.
Moreover as opposed to non-parametric methods such as kernel density estimates and nearest neighbor methods, adversarial learning suffers less from the curse of dimensionality, being able to model complex high-dimensional distributions  \citep{lopez2016revisiting,karras2017progressive}.

The second limitation of CGNN is a scalability issue w.r.t. the number of variables, due to the greedy search exploration in the space of DAGs, as all generative networks modeling the causal mechanisms in the causal graph must be retrained when a new graph structure is evaluated. SAM tackles this second issue by using an unified  framework for structure optimization, inspired by~\citep{Dag-no-tears}, where the mechanisms and the structure are simultaneously learned within a DAG learning framework. 


==> SAM_section_4.tex <==
%%%%%%%%%%%%%%% Je m'arrete ici

\section{Structural Agnostic model \label{sec:practical}}


As said, the {\em Structural Agnostic Model} (SAM) implements the above proposed settings, minimizing the global score (Eq.  (\ref{eq:global_score})). It addresses its optimization challenges using three original algorithmic choices: 
\begin{enumerate}
    \item Firstly, the space of admissible causal mechanism is not explicitly restricted, and each Markov kernel is modelled as a conditional generative neural network  \citep{mirza2014conditional}. All $d$ Markov kernels are learned in parallel, enforcing the scalability of the approach up to thousands of variables (see section \ref{sec:benchmarks}).
    \item Secondly, the conditional likelihood scores attached with each Markov kernel are approximated and optimized using an adversarial neural network. This approach does not require any assumption about the true distribution $p$ of the data (such as the Gaussianity of noise).
    \item Lastly, the combinatorial optimization issues related with finding a DAG are avoided as follows. On one hand, 
    an acyclicity constraint inspired from \cite{Dag-no-tears} is added to the learning criterion (Eq. (\ref{eq:global_score})), to learn a DAG by solving a continuous optimization problem (section \ref{sec:acyclicity_constraint}). 
    On the other hand, a Bernoulli reparametrization trick  \citep{maddison2016concrete,jang2016categorical} is used to simultaneously optimize the structure of the model (i.e. the $\a_j$'s) and the causal mechanisms (i.e. parameters $\theta_j$), using stochastic gradient descent. 
\end{enumerate}

These algorithmic choices are presented in the next three subsections. 


\subsection{Modeling each Markov kernel with a conditional generative neural network \label{sec:causal_gen}}

In order to model each Markov kernel $q_j(x_j | \mathbf{x}, \a_j, \btheta_j)$, each causal mechanism $\hat{f_j}$  is implemented as a H-hidden layer neural network, with $n_h$ nodes at the $h$-th hidden layer for $h = 1, ...,H$. The input is of dimension $n_0 = d + 1$, the output is of dimension $n_{H+1} = 1$. The mathematical expression of each deep neural network is given by:

\begin{equation}
   \begin{aligned}
    \hat{X}_j &= \hat{f}_j(\mathbf{X},E_j) \\
    &= L_{j,H+1} \circ \sigma \circ L_{j,H} \circ \dots \circ \sigma \circ L_{j,1}([\mathbf{a_j} \odot \mathbf{X},E_j])
    \label{eq:fcm_neural}
\end{aligned} 
\end{equation}

where $\mathbf{a_j} \odot \mathbf{X}$ corresponds to the element wise product between the two vectors $\mathbf{a_j}$ and $\mathbf{X}$, and $E_j$ is a Gaussian noise variable with zero mean and unit variance. $L_{j,h} : \mathbb{R}^{n_{h-1}} \rightarrow \mathbb{R}^{n_h}$ is an affine linear map defined by $L_{j,h}(\mathbf{x}) = \mathbf{W}_{j,h} \cdot \mathbf{x} + \mathbf{b}_{j,h}$ for given $n_h \times n_{h-1}$ dimensional weight matrix $\mathbf{W}_{j,h}$ (with coefficients $\{w^{j,h}_{k,l}\}_{1 \leq k \leq n_h \atop 1 \leq l \leq n_{h-1}}$), $n_h$ dimensional bias vector $\mathbf{b}_{j,h}$ (with coefficients $\{b^{j,h}_{k}\}_{1 \leq k \leq n_h}$) and $\sigma : \mathbb{R}^{n_h} \rightarrow ]-1,1[^{n_h}$  the element-wise nonlinear activation map defined by $\sigma(\mathbf{z}) := (tanh(z_1),...,tanh(z_{n_h}))^{T}$. We denote by $\theta_j$, the set of all weight matrices and bias vector of  the neural network modeling the $j$-th causal mechanism $\hat{f_j}$: $\theta_j := \{ (\mathbf{W}_{j,1}, \mathbf{b}_1), (\mathbf{W}_{j,2}, \mathbf{b}_2), \dots, (\mathbf{W}_{j,{H+1}}, \mathbf{b}_{H+1})\}$.

% \begin{equation}
%   \begin{aligned}
%     X_j &= \hat{f}_j(\mathbf{X},E_j) \\
    
%     &= \sum_{k=1}^{n_h} m_{j,k} \phi_{j,k}(\mathbf{X},E_j) + m_{j,0}\\
%     \mbox{with~}  \phi_{j,k}(\mathbf{X},E_j) &= tanh \left( \sum_{i=1}^d W_{j,i} a_jX_j + W_{j,0} + W_{j,d+1} E_j \right)
% %              &= m_j^\top \tanh \left( W_j^\top (\a_j \odot \mathbf{X}) + n_j E_j + b_j \right) \odot \z_j + \beta_j,
%     \label{eq:fcm_neural}
% \end{aligned} 
% \end{equation}


%\michele{ici modifié pour avoir notations homogènes; $n_j$ faisait penser à un entier, $\beta_j$ est homogène à un $m$}
%\olivier{ok}


\begin{figure}[H]
    \centering
    \input{generator_fig.tex}
    \caption{Diagram of the conditional generative neural network modeling the causal mechanism  $\hat{X}_j = \hat{f}_j(\mathbf{X},E_j)$.}
    \label{fig:generator_fig}
\end{figure}




% Each neural network $\hat{f}_j$ thus encodes a generative model $q_j(x_j | x_{\Pahat{j}}, \btheta_j)$ of $X_j$ conditionally to variables in $X_{\Pahat{j}}$, with $\Pahat{j} = \{i \in [1,\ldots,d] ~s.t.~ a_{i,j} = 1 \}$. 
At every evaluation of noise variable $E_j$, a value is drawn anew from distribution $\mathcal{N}(0, 1)$.  All the noise variables $E_j$ for $j \in \llbracket 1, d \rrbracket$ are drawn from independent distributions.



%By construction in the SAM model, each generated variable $\hat{X}_j$ only depends on  $X_{\Pahat{j}}$. 

 




%\diviyan{Added small details, maybe clarify a bit more.\\
%Michele: say what sigma is (tanh ?).}
%\olivier{yes}

\paragraph{Parallel computation with three dimensional tensor operations}

For a better computational efficiency on GPU devices, the $d$ causal mechanisms $\hat{f}_j$ for $j=1,..,d$ (Equation (\ref{eq:fcm_neural})) are computed in parallel with three dimensional tensor operations by stacking all the generative neural networks along a third dimension. The generation of each $\hat{X}_j$ is independent from the generations of the other variables $\hat{X}_i$, with $i=0, \dots,j-1,j+1,\dots,d$. As these $d$ variable generations are independent calculation, they can be done in parallel. 

%Indeed, we can directly compute the output vector $ \hat{\mathbf{X}} = 
Specifically, the output vector $ \hat{\mathbf{X}} = 
(\hat{X_1},\dots,\hat{X_d})$ is computed from $\mathbf{X}$ as:

\begin{equation}
    \hat{\mathbf{X}} = L_{H+1} \circ \sigma \circ L_{H} \circ \dots \circ \sigma \circ L_{1}([\mathbf{A} \odot \mathbf{\bar{X}},\mathbf{E}]),
    \label{eq:parallel_fcm_neural}
\end{equation}

where $A$ denote the structural gate matrix of size $d \times d$ (the adjacency matrix of the graph) formed by the $d$ vectors $\mathbf{a_j}$ for $j=1,..,d$, and $\mathbf{\bar{X}}$ corresponds to a matrix formed by $d$ replications of the vector $\mathbf{X}$.\\ We denote by $[\mathbf{A} \odot \mathbf{\bar{X}},\mathbf{E}]$ the matrix of size $ (d+1) \times d$ and resulting from the concatenation between the $d \times d$ matrix $\mathbf{A} \odot \mathbf{\bar{X}}$ and the $d$ dimensional noise vector $\mathbf{E}=(E_1,\dots,E_d)$. $L_{h} : \mathbb{R}^{d \times (n_{h-1})} \rightarrow \mathbb{R}^{d \times n_h}$ is the affine linear map defined by $L_{h}(\mathbf{x}) = \mathbf{\bar{W}}_{h} \cdot \mathbf{x} + \mathbf{\bar{b}}_h$ with the  $d \times n_h \times n_{h-1}$ dimensional weight tensor $\mathbf{\bar{W}}_h$ (corresponding to the aggregation of the $d$ matrices $\mathbf{W}_{j,h}$ for $j=1,..,d$) and the $d \times n_h$ dimensional bias matrix $\mathbf{\bar{b}}_h$ (aggregation of the $d$ vectors $\mathbf{b}_{j,h}$ for $j=1,..,d$).





%For notational simplicity, each $\hat{f}_j$ is associated with a parameter vector $\btheta_j = (\theta_{j,1}, \ldots, \theta_{j,p_j})$ (including vectors ${\bf m}_j$ and $W_{j, \cdot}$ but excluding the $\a_j$ and $\z_j$ gates). 

%Each causal mechanism is written $\hat{f}_j^{\theta_j,a_j,z_j}$, with $\theta = (\theta_1, \ldots, \theta_d)$. 
%\michele{Notations: $\theta$ ne peut pas etre $d$-dimensionel si $d$ est le nombre de var.}
%\diviyan{j'ai rajouté la dimension j à  $\theta_1j, \ldots, \theta_pj$}




% Moreover, as the conditional densities $q(x_j | x_{\Pahat{j}}, \btheta_j, \z_j)$ can be computed independently, $$K(q(\x,\widehat{\mathcal{G}},\theta,Z)) \overset{+}{=} \sum_{j=1}^d K(q(x_j | x_{\Pahat{j}}, \btheta_j, \z_j)).$$

% The normalized MDL for a candidate graph $\widehat{\mathcal{G}}$  (Eq. (\ref{eq:MDL})) thus is rewritten as a sum of $d$ local scores:

% \begin{equation} \label{eq:glob_score_decomposbale}
% MDL(\widehat{\mathcal{G}},\theta^*, D) 
%  =   \underset{\theta,Z}{min} \left[\underbrace{\frac{1}{n} \sum_{j=1}^d  K(q(x_j | x_{\Pahat{j}}, \theta_j, \z_j))}_\textrm{model complexity} + \ \underbrace{\frac{1}{n} \sum_{j=1}^d \sum_{\ell = 1}^{n} \text{log}\  \frac{1}{q(x^{(\ell)}_j | x^{(\ell)}_{\Pahat{j}}, \btheta_j, \z_j)}}_\textrm{fit loss}  \right]
% \end{equation}
% with $\theta^*$ the optimal set of parameters for the considered model.




\subsection{SAM learning criterion \label{SAM_criterion}}



%\isabelle{Cette section est trop longue, on perd le fil. Je mettrais tout ca en appendice. Je mentionnerai juste: In this section, we derive a principled loss function to be optimized by the SAM algorithm, based on the MDL principle. Following the arguments developed in details in appendix, we arrive at the following formula [give the formula number, (21) or whatever. This formula, whose entire justification is given in appendix, has the simple following intuitive interpretation: term 1 blah blah, term 2 blah blah}
%\michele{Ok, j'essaye d'implémenter la suggestion d'Isabelle}

% This section derives a principled loss function from the model complexity and data fitting terms, defining SAM learning criterion. 

This section describes how SAM tackles the optimization problem defined in Eq. (\ref{eq:global_score}), assessing each  candidate DAG $\widehat{\mathcal{G}}$ as:


 \begin{equation*}
 S^n(\widehat{\mathcal{G}},\theta, D) 
 :=  - \underbrace{\frac{1}{n} \sum_{j=1}^d \sum_{\ell = 1}^{n} %\frac{1}
 {\text{log}\  q_j(x^{(\ell)}_j | \mathbf{x}_{-j}^{(\ell)}, \a_j, \btheta_j)}}_\textrm{fit loss} + \underbrace{  \lambda_S  \sum_{j=1}^d \sum_{i=1}^d a_{i,j} +  \lambda_F \sum_{j=1}^d  \|\theta_j\|_F}_\textrm{model complexity}
 \end{equation*}


\paragraph{Model complexity}
\def\Ghat{\mbox{$\widehat{\mathcal{G}}$}}

The complexity of each causal mechanism $\hat{f}_j$ is the sum of two terms, with respectively regularization weights $\lambda_S >0 $ and  $\lambda_F >0$\,:

\begin{itemize}
    \item the \textit{structural} complexity measured by the $L_0$ norm of the structural gate $\a_j$, representing the number of parents of $X_j$.
    \item the \textit{functional} complexity $\|\theta_j\|_F$ of the causal mechanism, measured as the  Frobenius norm of the weight matrix, 
    providing a good measure of the
    functional complexity of a deep neural network
    \citep{neyshabur2017exploring}. More precisely, 
    \begin{equation}
        \|\theta_j\|_F = \sum_{h=1}^{H+1} \|\mathbf{W}_{j,h}\|_F + \sum_{h=1}^{H+1} \|\mathbf{b}_{j,h}\|_F,
    \end{equation}
    with $\|\mathbf{W}_{j,h}\|_F = \sqrt{\sum_{1 \leq k \leq n_h \atop 1 \leq l \leq n_{h-1}} |w^{j,h}_{k,l}|^2}$ and $\|\mathbf{b}_{j,h}\|_F = \sqrt{\sum_{1 \leq k \leq n_h} |b_k^{j,h}|^2}.$
\end{itemize}



 \paragraph{Data fitting loss\label{sec:fit_term}}

  When the number $n$ of samples goes to infinity, 
  the data fitting term goes to data log-likelihood expectation under the sought generative distribution. With same notations as in section \ref{sec:problem}:

\begin{equation}
    \lim_{n\to\infty} \frac{1}{n} \sum_{\ell = 1}^{n} %\frac{1}
    {\text{log}\  q_j(x^{(\ell)}_j | \mathbf{x}_{-j}^{(\ell)}, \a_j, \btheta_j)} 
 =  \  \mathbb{E}_{p(\mathbf{x})} \ \text{log}\ {q_j(x_j | \mathbf{x}_{-j}, \a_j, \btheta_j)} \\
\end{equation}

 
Let us denote $\tilde{\mathbf{X}} = \left[X_1,\ldots X_{j-1},\hat{X}_j, X_{j+1}\dots, X_d \right]$, the vector of $d$ variables, where the only variable $\hat{X}_j$ is generated from model $\hat{f}_j$, all other variables being the observed variables. We denote  $\tilde{q_j}(\tilde{\mathbf{X}})$ (or simply $\tilde{q_j}$)  its joint distribution and 
$\tilde{q_j}(x_j,\x_{-j},\a_j, \btheta_j)$ its joint density.  By construction,  $\tilde{q_j}(x_j,\x_{-j},\a_j, \btheta_j) = p(\x_{-j})q_j(x_j|\x_{-j},\a_j, \btheta_j)$.

Therefore, we have:

% \def\X{\mbox{\bf X}}
\begin{align}
\lim_{n\to\infty} \frac{1}{n} \sum_{\ell = 1}^{n} %\frac{1}
{\text{log}\  q_j(x^{(\ell)}_j | \mathbf{x}_{-j}^{(\ell)}, \a_j, \btheta_j)}   
&= \mathbb{E}_{p(\mathbf{x})} \ \text{log}\  \frac {q_j(x_j|\x_{-j},\a_j,\btheta_j)}{p(x_j|\x_{-j})} + \mathbb{E}_{p(\mathbf{x})} \ \text{log}\  p(x_j|\x_{-j}) \\
&= \mathbb{E}_{p(\mathbf{x})} \ \text{log}\  \frac {q_j(x_j|\x_{-j},\a_j,\btheta_j)p(\x_{-j})}{p(x_j|\x_{-j})p(\x_{-j})} + \mathbb{E}_{p(\mathbf{x})} \ \text{log}\  p(x_j|\x_{-j}) \\
&= -\mathbb{E}_{p(\mathbf{x})} \ \text{log}\  \frac{p(\mathbf{x})} {\tilde{q_j}(x_j,\x_{-j},\a_j,\btheta_j)} + \mathbb{E}_{p(\mathbf{x})} \ \text{log}\  p(x_j|\x_{-j}) \\
 & =  - D_{KL}[p \, \Vert \, \tilde{q_j}] + H(X_j|\X_{-j}),
% \label{eq:KL_score}
\end{align}


\noindent with $D_{KL}[p \, \Vert \, \tilde{q_j}] =  \mathbb{E}_{p(\mathbf{x})} \ \text{log}\  \frac{p(\mathbf{x})} {\tilde{q_j}(x_j,\x_{-j},\a_j,\btheta_j)}$  the Kullback-Leibler divergence between  the distributions  $p(\mathbf{X})$  and  $\tilde{q_j}(\tilde{\mathbf{X}})$, and  $H(X_j|\X_{-j})$ the constant, domain-dependent entropy of $X_j$ conditionally to  $\X_{-j}$ (neglected in the following). 

Therefore, the optimization task needs to estimate the quantity $D_{KL}[p \, \Vert \, \tilde{q_j}]$ for $j = 1, \dots, d$.

As the estimation of each $D_{KL}[p \, \Vert \, \tilde{q_j}]$ is intractable in practice for continuous data, we estimate instead its variational dual representation as $f$-divergence. Let $\mathcal{T}$ be an arbitrary class of functions $T: \mathbb{R}^{d} \rightarrow \mathbb{R}$. For two distributions $p$ and $q$ defined over $\mathbb{R}^{d}$, \cite{nguyen2010estimating} establish the following lower bound (tight for sufficiently large families $\mathcal{T}$):

\begin{equation}
D_{KL}[p \, \Vert \, q] \geq \underset{T \in \mathcal{T}}{\text{sup}}\  \mathbb{E}_{p(\mathbf{x})}[T(\mathbf{x})] - \mathbb{E}_{ q(\mathbf{x})}[e^{T(\mathbf{x}) -1}],
\end{equation}

The \textit{f-gan} approach proposed by \cite{nowozin2016f} relies on defining $\mathcal{T}$ as the family of functions $T_{\omega} : \mathbb{R}^{d} \rightarrow \mathbb{R}$ parameterized by a deep neural network with parameter $\omega \in \Omega$, and minimizing the lower bound on  $D_{KL}[p \, \Vert \, q]$ defined as: 

\begin{equation}
D_{KL}[p \, \Vert \, q] \geq \underset{\omega \in \Omega}{\text{sup}}\ \mathbb{E}_{p(\mathbf{x})}[T_{\omega}(\mathbf{x})] - \mathbb{E}_{q(\mathbf{x})}[e^{T_{\omega}(\mathbf{x}) -1}]
\label{eq:f-gan}
\end{equation}

Taking inspiration from the \textit{f-gan}, SAM simultaneously trains the $d$ neural networks $\hat{f}_j$, as follows. For $\ell = 1, \ldots, n$, let $\x^{(\ell)}_{-j}$ be defined from $\x^{(\ell)}$ by taking all its coordinates but the $j$-th, let $e^{(\ell)}_j$ be drawn from Gaussian $\mathcal{N}(0, 1)$, and let scalar $\hat{x}^{(\ell)}_j$ be computed from $\hat{f}_j$ (Eq.~\eqref{eq:fcm_neural}) as:
$$\hat{x}^{(\ell)}_j = \hat{f}_j(\x^{(\ell)}_{-j},e^{(\ell)}_j)$$
Let the pseudo-sample $\tilde{\x}^{(\ell)}_j$ be defined from $\x^{(\ell)}$ by setting its $j$-th coordinate to $\hat{x}^{(\ell)}_j$, and let the dataset $\tilde{D}_j$ include all pseudo-samples $\tilde{\x}^{(\ell)}_j$ for $\ell = 1\ldots n$. 
For $j = 1, \ldots, d$, let $T^j_{\omega}$ be trained to discriminate between the dataset $D$ drawn from the original $p(\mathbf{X})$ distribution,  and  the dataset $\tilde{D}_j$ drawn from $\tilde{q_j}(\tilde{\mathbf{X}})$. After Eq. (\ref{eq:f-gan}),

\begin{multline}\label{eq:KL}
 D_{KL}[p \, \Vert \, \tilde{q_j}] \geq   \underset{\omega \in \Omega_j}{\text{sup}}\ \lim_{n\to\infty} \Bigg( \frac{1}{n} \sum_{\ell=1}^{n}   T^j_{\omega}(\x^{(\ell)}) + \frac{1}{n} \sum_{\ell=1}^{n} [\, -\exp(T^j_{\omega}(\tilde{\x_j}^{(\ell)}) - 1) \,]\Bigg)   
\end{multline}

One could indeed use $d$ different adversarial neural networks $T^j_{\omega}$ to estimate 
each $D_{KL}[p \, \Vert \, \tilde{q_j}]$. However, the use of a single discriminator $T_{\omega}$ to achieve the $d$ discrimination tasks is both more computationally efficient, and more stable: it empirically avoids the gradient vanishing 
phenomena that were observed when solving separately the $d$ min-max optimization problems with $d$ different discriminators.

By using a single shared discriminator $T_{\omega}$, it comes: 

\begin{align}
\sum_{j=1}^d D_{KL}[p \, \Vert \, \tilde{q_j}] & \geq \sum_{j=1}^{d} \underset{\omega \in \Omega}{\text{sup}}\ \lim_{n\to\infty}  \frac{1}{n}  \left (
\sum_{\ell=1}^{n}   T_{\omega}(\x^{(\ell)}) +  \sum_{\ell=1}^{n} [\, -\exp(T_{\omega}(\tilde{\x_j}^{(\ell)}) - 1)] \right ) \\
& \geq  \underset{\omega \in \Omega}{\text{sup}}\ \lim_{n\to\infty} \left( \frac{d}{n} 
\sum_{\ell=1}^{n} T_{\omega}(\x^{(\ell)}) + \frac{1}{n}  \sum_{j=1}^{d} \sum_{\ell=1}^{n} [\, -\exp(T_{\omega}(\tilde{\x_j}^{(\ell)}) - 1)]\right)
\label{eq:kl_fgan2}    
\end{align}

Accordingly, SAM tackles the minimization of the empirical approximation of the above lower bound on  $\sum_{j=1}^{d} D_{KL}[p \, \Vert \, \tilde{q_j}]$,  defined as: 

\begin{equation}
 \underset{\omega \in \Omega}{\text{sup}}\ \left( \frac{d}{n} 
\sum_{\ell=1}^{n} T_{\omega}(\x^{(\ell)}) + \frac{1}{n}  \sum_{j=1}^{d} \sum_{\ell=1}^{n} [\, -\exp(T_{\omega}(\tilde{\x_j}^{(\ell)}) - 1)]\right)
\end{equation}


% \paragraph{Evaluation of the global loss min-max penalized optimization problem with SAM}
  \paragraph{Evaluation of the global penalized min-max loss optimization problem.}
  
Eventually, SAM is trained to solve the min-max penalized optimization problem defined as:\footnote{Generator $\hat{f}_j$ is written with superscripts $\theta_j$ and $\mathbf{a}_j$ to indicate that it depends on both parameters $\theta_j$ and  $\mathbf{a}_j$.}

\begin{multline}
L^n(\widehat{\mathcal{G}}^*,\theta^*, D) = \underset{A,\theta}{\text{min}} \\
\left( 
\underbrace{\lambda_S \sum_{i=1,j=1}^d a_{i,j} + \lambda_F \sum_{j=1}^d  \|\theta_j\|_F}_\textrm{model complexity}  + \underbrace{\underset{\omega \in \Omega}{\text{sup}}\ \left( \frac{d}{n} 
\sum_{\ell=1}^{n} T_{\omega}(\x^{(\ell)}) + \frac{1}{n}  \sum_{j=1}^{d} \sum_{\ell=1}^{n} [\, -\exp(T_{\omega}(\hat{f}^{\theta_j,\mathbf{a}_j}_j(\x^{(\ell)},e^{(\ell)}_j), {\x}^{(\ell)}_{- j}) - 1)]\right)}_\textrm{fit loss} \right)  
\label{eq:global_score_eval}
\end{multline}
%J'ai mis sur une seule ligne pour avoir les parenthèses de la bonne hauteur.

where the minimization is carried over the parameters $\btheta = (\btheta_1, \ldots, \btheta_d)$ of the $\hat{f}_j$ and over the matrix $A = (a_{i,j})$  representing the structural gates. 




\begin{figure}[H]
    \centering
    \input{sam_fig.tex}
    \caption{A four-variable example: diagram of the SAM structure for variables $X_1,\ldots,X_4$}
    \label{fig:sam_fig}
\end{figure}


Figure \ref{fig:sam_fig} illustrates a 4-variable SAM: on the left are the four generators  corresponding to the causal mechanisms  $\hat{f}_j^{\theta_j,a_j}$, for $j = 1 \ldots 4$. On the right is the shared neural network discriminator $T_{\omega}$ evaluating the global fit loss corresponding to the sum of the estimated fit terms  $D_{KL}[p \, \Vert \, \tilde{q_j}]$ for $j = 1 \ldots 4$. 


\subsection{Enforcing the acyclicity of the causal graph\label{sec:acyclicity_constraint}}
Note that Equation (\ref{eq:global_score_eval}) does not ensure that the optimal $\widehat{\mathcal{G}}$ be a DAG: the sparsity constraint on \Ghat\ through the model complexity term (minimizing $\|\a_j\|_0$) leads to independently identify the Markov blanket of each variable $X_j$, selecting all causes, effects and spouses thereof \citep{yu2018unified}. 

In order to ensure that the solution is a DAG and avoid the associated combinatorial optimization issues (section \ref{sec:soa}),
%. Furthermore, as the $\widehat{\mathcal{G}}$ assessment depends on the trained discriminator $T_\omega$, this adversely affects the comparison of different graph structures. 
it is proposed to augment the learning criterion with an acyclicity term inspired from \cite{Dag-no-tears}. Letting $A$ denote the structural gate matrix (the adjacency matrix of the graph), $\widehat{\mathcal{G}}$
is a DAG iff
% In appendix
%\footnote{Other DAG characterizations could be considered, e.g. $A^d = 0$ or $\sum_{k=1}^d  \text{tr}\ A^k = 0$. These however appear to be impractical for numerical reasons. Indeed, without any re-weighting of the number of cycles of size $k$ by $k!$, the entries of $A^k$ can easily exceed machine precision for even small values of $d$, which makes both function and gradient evaluations highly unstable  \citep{zheng2018dags}.} 
$$\sum_{k=1}^d \frac{\text{tr}\ A^k}{k!} = 0.$$

Accordingly, the learning criterion is augmented with an acyclicity term, with:


\begin{equation}
 \begin{aligned}
L^n(\widehat{\mathcal{G}}^*,\theta^*, D)  = \underset{A,\theta}{\text{min}} \ \underset{\omega \in \Omega}{\text{max}} \ & \Bigg( \frac{1}{n} \sum_{\ell=1}^{n}  \sum_{j=1}^d  [\, T_{\omega}(\mathbf{x}^{(\ell)}) -\exp(T_{\omega}(\hat{f}^{\theta_j,\mathbf{a}_j}_j(\x^{(\ell)},e^{(\ell)}_j), {\x}^{(\ell)}_{- j}) - 1)] \\ & +  \lambda_S \sum_{i,j} a_{i,j} + \lambda_F \sum_{j}  \|\theta_j\|_F  + \lambda_D \sum_{k=1}^d\frac{\text{tr}\ A^k}{k!} \Bigg),
\label{eq:global_loss}
\end{aligned}
\end{equation}

%\michele{Le fait qu'on ait 1/n partout sauf devant le terme d'acyclicité - alors qu'il suffirait de le rentrer ds $\lambda_D$ - et le fait qu'on minimise, donc à constant mult. près, continue à me gêner.}
%\diviyan{Le terme d'acyclicité, (avec le $\lambda_d$) est le seul terme qui ne dépend pas des données, mais de la structure du graphe en lui meme. tous les autres scores évoluent en fonction du nombre de points donnés en input. }
%\olivier{On minimise à une constante multiplicative près. Empiriquement ça donne de meilleure résultats d'introduire cette contrainte de DAG de façon progressive. Si on le contraint trop vite à choisir une orientation le modèle se trompe souvent.}
with $\lambda_D \geq 0$ a penalization weight.\footnote{In practice, $\lambda_D$ is small at the initialization and increases along time; in this way, the structural penalization term $\lambda_S \sum_{i,j} a_{i,j}$ can operate and prune the less relevant edges before considering the DAG constraint. }

This acyclicity constraint creates a coupling among the $d$ feature selection problems, implying that at most one arrow between pairs of variables can be selected,
%(removing the 2-cycles), 
and more generally leading to remove effect variables from the set of parents of any  $X_i$; the removal of effect variables in turn leads to removing spouse variables as well (section \ref{sec:structural_loss}).  

As the use of the $L_0$ norms of the vectors $\a_j$, if naively done, could entail computational issues (retraining the network from scratch for every new graph structure or neural architecture), an approach based on the Bernoulli reparameterization trick is proposed to 
end-to-end train the SAM architecture and weights using stochastic gradient descent \citep{srivastava2014dropout,louizos2017learning} and the Binary Concrete relaxation approach \citep{maddison2016concrete,jang2016categorical}. This solution corresponds to a learned dropout of edges  of the neural network.
 
 Overall, the optimization of the learning criterion in Equation (\ref{eq:global_loss}) with the acyclicity and sparsity constraints defines the \textit{Structural Agnostic Model} SAM (Alg. \ref{algo:SAM}, Figure \ref{fig:sam_fig}).
%  \textcolor{blue}{ For a better clarity of the algorithm, the computation and training of each of the $d$ conditional generative neural networks with loops from 1 to d, but 
 
 

\begin{algorithm}[h!]
\caption{The Structural Agnostic Modeling Algorithm}
\noindent\begin{minipage}{\textwidth}
\renewcommand\footnoterule{}                  %% This line should come here.

\label{algo:SAM}
\begin{algorithmic}

\FOR{number of iterations} 

%\STATE \FOR{j = 1, \ldots, d} 
\STATE $\bullet$ \textbf{Forward phase} :
\STATE \quad i)  sample the structural gate matrix $A$: for $i,j = \llbracket 1, d \rrbracket \times \llbracket 1, d \rrbracket$,  $a_{i,j} = \text{cst}(H (l_{i,j} + a'_{i,j})) - \text{cst}(\text{sigmoid} (l_{i,j} + a'_{i,j})) + \text{sigmoid} (l_{i,j} + a'_{i,j})$ with $l_{i,j}$ drawn from logistic  distribution and $H$ the Heavyside step function.
% Avoid: a everywhere, it's confusing.
$^{(*)}$ 
%\footnote{$\text{cst}()$ represents the copy by value operator transforming the input into a constant with the same value but zero gradient. With this trick the value of  $a_{i,j}$ is equal to $H (l_{i,j} + a'_{i,j})$ (forward pass) but its gradient w.r.t $a'_{i,j}$ is equal to $\nabla_{a'_{i,j}} \text{sigmoid}(l_{i,j} + a'_{i,j})$ (backward pass).}. 
$A'$ denotes the matrix with the $a'_{i,j}$ coefficients.
%\STATE $\bullet$ sample the functional gate vector $\z_j$: for $h = 1, \ldots, n_h$, $z_{h,j} = \text{cst}(H (l_{h,j} + z'_{h,j})) - \text{cst}(\text{sigmoid}(l_{h,j} + z'_{h,j})) + \text{sigmoid}(l_{h,j} + z'_{h,j})$ with $l_{h,j}$ drawn from logistic distribution.
\STATE \quad ii)  sample noise vector, $\mathbf{e^{(\ell)}} = (e^{(\ell)}_1, \dots,e^{(\ell)}_d)$ from multivariate normal distribution ${\cal N}(\mathbf{\mu},\mathbf{\Sigma})$ with $\mathbf{\mu} = (1,\dots,1)$ and  $\mathbf{\Sigma} = I$ (independent noise variables).

\STATE \quad iii) generate $n$ samples   $\{\hat{\x}^{(\ell)}\}_{l=1}^{n}= \{(\hat{x}_1^{(\ell)}, \dots, \hat{x}_d^{(\ell)})\}_{l=1}^{n}$ such that for $\ell = 1 \ldots,n$ :

\begin{align*}
 \hat{\x}^{(\ell)} &=  (\hat{f}^{\theta_1,\mathbf{a}_1}_1(\x^{(\ell)},e^{(\ell)}_1), \dots, \hat{f}^{\theta_d,\mathbf{a}_d}_d(\x^{(\ell)},e^{(\ell)}_d)) \\
     &= L_{H+1} \circ \sigma \circ L_{H} \circ \dots \circ \sigma \circ L_{1}([A \odot {\bar{\x}}^{(\ell)},\mathbf{e}^{(\ell)}]), %\hat{f}_j^{\theta_j,a_j}({\x}^{(\ell)},e^{(\ell)}_j) \\
%    &= m_j^\top \tanh \left( W_j^\top (\a_j \odot \x^{(\ell)}) + n_j E_j + b_j \right) \odot \z_j + \beta_j
%&= \sum_{k=1}^{n_h} m_{j,k} tanh \left( \sum_{i=1}^d W_{j,i} a_jX_j + W_{j,0} + W_{j,d+1} E_j \right) + m_{j,0}\\
\end{align*}
where $\bar{\x}^{(\ell)}$ corresponds to the matrix formed by $d$ copies of the vector $\x^{(\ell)}$.

%\ENDFOR
\STATE $\bullet$ \textbf{Backward phase} :
\STATE \quad i) update the discriminator by ascending its stochastic gradient: $$\nabla_{\omega}  \left[\frac{d}{n} \sum_{\ell=1}^{n} T_{\omega}(\x^{(\ell)})  \ + \frac{1}{n} \sum_{j=1}^{d} \sum_{\ell=1}^{n} [\, -\exp(T_{\omega}(\hat{x}^{(\ell)}_j, {\x}^{(\ell)}_{- j}) - 1) \,] \right]$$

\STATE \quad ii)  update the all the conditional generators by descending their stochastic gradients w.r.t the set of parameters $\theta = (\theta_1, \dots, \theta_d)$ and the set of parameters $a_{i,j}$ of the structural gates adjacency matrix $A$ : 
\begin{align*}
    \nabla =& \nabla_{\theta} \left[ \frac{1}{n} \sum_{j=1}^{d} \sum_{\ell=1}^{n} [\, -\exp(T_{\omega}(\hat{f}^{\theta_j,\mathbf{a}_j}_j(\x^{(\ell)},e^{(\ell)}_j), {\x}^{(\ell)}_{- j}) - 1) \,] +  \lambda_F \sum_{j}  \|\theta_j\|_F \right]\\
    &+ \nabla_{A'} \left[ \frac{1}{n} \sum_{j=1}^{d} \sum_{\ell=1}^{n} [\, -\exp(T_{\omega}(\hat{f}^{\theta_j,\mathbf{a}_j}_j(\x^{(\ell)},e^{(\ell)}_j), {\x}^{(\ell)}_{- j}) - 1) \,] + \lambda_S \sum_{i,j} a_{i,j} + \lambda_D \sum_{k=1}^d\frac{\text{tr}\ A^k}{k!} \right] \\
    %&+ \nabla_{\z'_j} \left[ \frac{1}{n} \sum_{\ell=1}^{n} [\, -\exp(T_{\omega}(\tilde{x}^{(\ell)}_j, {\x}^{(\ell)}_{- j}) - 1) \,] + \frac{\lambda_F}{n} \sum_{j,h} z_{h,j} \right]
\end{align*}
\ENDFOR
\STATE Return $A$ and $\theta$\\
{\footnotesize $^{(*)}$: $\text{cst}()$ represents the copy by value operator transforming the input into a constant with the same value but zero gradient. With this trick the value of  $a_{i,j}$ is equal to $H (l_{i,j} + a'_{i,j})$ (forward pass) but its gradient w.r.t $a'_{i,j}$ is equal to $\nabla_{a'_{i,j}} \text{sigmoid}(l_{i,j} + a'_{i,j})$ (backward pass).}

\end{algorithmic}
%\footnotetext{}
\end{minipage}
\end{algorithm}
%\michele{On peut pas simplifier ce "the set of parameters $\a'_j$ of the structural gates $\a_j$": on prend la dérivée par rapport à $\a_j$, et la valeur de la dérivée au point ou on est... Le fait de distinguer les deux me parait confusant.}
%\olivier{Je trouve ça plus clair de distinguer les deux jeux de paramètres. C'est vraiment comme ça que fonctionne l'algo. On est obligé de faire cette approximation avec la sigmoid en passe backward pour que le gradient soit informatif. }

% \subsection{Candidate model } 

% The goal in this paper is to uncover the functional causal model $(\mathcal{G}, f)$ (Eq.  (\ref{eq:fcm})) defining the data joint distribution from a $n$-sample thereof. 





==> SAM_section_7.tex <==
\section{Discussion and Perspectives \label{sec:conclusion}}
The main contribution of the paper is to propose a new causal discovery method, exploiting both structural independence and distributional asymmetries through optimizing structural and functional criteria. This framework is implemented in the SAM algorithm,\footnote{Available at \url{https://github.com/Diviyan-Kalainathan/SAM}.} leveraging the 
%non-parametric 
representational 
power of Generative Adversarial Neural networks (GANs) to 
%capture a  non-parametric
learn a generative model 
using stochastic gradient descent,
and enforcing the discovery of 
%acyclic causal graphs through sparsity and 
%Euclidian 
%Euclidean norm regularizations. 
sparse acyclic causal graphs through adequate regularization terms.


The choices made in the construction of the model (joint log-likelihood estimation of the conditional distributions with the use of an adversarial f-gan neural network; usage of structural, functional and acyclicity constraints) are supported by a theoretical analysis. 


In the general case, the identifiability of the causal graph with neural networks as causal mechanisms remains an open question, left for further work. 
%However, extensive empirical evidence is gathered to show SAM's robustness
In practice, SAM robustness is supported by extensive empirical evidence 
across diverse synthetic, realistic and real-world problems, suggesting that SAM can be used as a powerful tool  for 
the practitioner in order to prioritize exploratory experiments when working on real data with no prior information about neither the type of functional mechanisms involved, nor the underlying data distribution. 

Lesion studies are conducted to assess whether and when it is beneficial to learn non-linear mechanisms and to rely on adversarial learning as opposed to MSE minimization.\\
As could have been expected, in particular settings SAM is dominated by algorithms specifically designed for  these settings, such as 
CAM~\citep{buhlmann2014cam} in the case of additive noise model and Gaussian process mechanisms, and GENIE3 when facing causal graphs with feedback loops for some networks. Nevertheless, SAM most often ranks first and always avoids catastrophic failures.  SAM has good overall computational efficiency compared to other non-linear methods as it uses an embedded framework for structure optimization, where the mechanisms and the structure are simultaneously learned within an end-to-end DAG learning framework.
 It can also easily be trained on a GPU device, thus leveraging on massive parallel computation power available to learn the DAG mechanisms and the adversarial neural network. SAM scalability is demonstrated on the {\em Network 1} of the DREAM5 challenge, obtaining very good performances with a relatively high number of variables (ca 1,500).

This work opens up four avenues for further research. An on-going extension regards the case of categorical and mixed variables, taking inspiration from discrete GANs \citep{hjelm2017boundary}. Another perspective is to relax the causal sufficiency assumption and handle hidden confounders, e.g. by introducing statistical dependencies between the noise variables attached to different variables \citep{rothenhausler2015backshift}, or creating shared noise variables \citep{janzing2018detecting} 
or proxies of confounders \citep{WangB21}.


A longer term perspective is to extend SAM to simulate interventions on target variables. 
Lastly, the case of causal graphs with cycles will be considered, leveraging the power of recurrent neural nets to define a proper generative model from a graph with feedback loops. 




==> generator_fig.tex <==
 \resizebox{.6\linewidth}{!}{
  \begin{tikzpicture}
  \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,minimum size=17pt,inner sep=0pt, draw=black]
    \tikzstyle{proba}=[rectangle, draw=black, minimum size=14pt, inner sep=0pt]
    \tikzstyle{input neuron}=[neuron];
    \tikzstyle{output neuron}=[neuron];
    \tikzstyle{hidden neuron}=[neuron];
    \tikzstyle{annot} = [text width=4em, text centered]
    \genj{1}{0}{1}
    %\gen{4}{0}{-4}
    %\dataset{1}{5.6}{.65}
    %\dataset{4}{5.6}{-4.35}
    %\foreach \coord in {1,...,3}
    %{\draw[fill=black] (0, \coord/2.5-4) circle (.02);
    %  \draw[fill=black] (-2.1, \coord/2.5-4) circle (.02);
    %  \draw[fill=black] (4.8, \coord/2.5-4) circle (.02);

    %}
    \foreach \coord in {1,...,3}
    {\draw[fill=black] (-1, \coord/5-.8) circle (.02);
      \draw[fill=black] (-1, \coord/5-2.95) circle (.02);
      \draw[fill=black] (-2.5, \coord/5-.8) circle (.02);
      \draw[fill=black] (-2.5, \coord/5-2.95) circle (.02);
    %  \draw[fill=black] (4.8, \coord/2.5-4) circle (.02);

    }
    %\nn{4}{9}{-1.5}
    %\draw[->, semithick] (5.6+1.8,.65-1.25) -- (8.5,-2.5);
    %\draw[->, semithick] (5.6+1.8,-4.35-1.25) -- (8.5,-4);
    %\tdataset{}{8.8}{2}
    \draw[brace, decoration={raise= .2cm}] (-.3, .9) -- (-1.7, .9);
    % \draw[brace, decoration={raise= .2cm}] (2.9, .9) -- (1.9, .9);
    \node[align=center] (label1) at (-1.1, 1.5) {Structural gates};
    %\node[align=center] (label2) at (2.4, 1.5) {Functional gates};
%\draw[brace, decoration={raise= .2cm}] (-1.3, -7.2) -- (-.7, -7.2);
    %\draw[brace, decoration={raise= .2cm}] (-.5, -7.4) -- (4.5, -7.4);
    %\draw[brace, decoration={raise= .2cm}] (5.5, -7.4) -- (7.6, -7.4);
    %\draw[brace, decoration={raise= .2cm}] (8.5, -7.4) -- (14, -7.4);
    % \node[align=center] (label3) at (2, -8) {Generators};
    % \node[align=center] (label4) at (6.5, -8) { $\mathcal{Q}$: Generated data};
    % \node[align=center] (label5) at (11.3, -8) {Discriminator};

    % \draw[brace, decoration={raise= .2cm}] (#2 + 1.8, #3) -- (#2, #3);
    % \draw[brace, decoration={raise= .2cm}] (#2 + 1.8, #3) -- (#2, #3);
    % \draw[brace, decoration={raise= .2cm}] (#2 + 1.8, #3) -- (#2, #3);

 \end{tikzpicture}
}


==> sam_fig.tex <==
 \resizebox{\linewidth}{!}{
  \begin{tikzpicture}
  \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,minimum size=17pt,inner sep=0pt, draw=black]
    \tikzstyle{proba}=[rectangle, draw=black, minimum size=14pt, inner sep=0pt]
    \tikzstyle{input neuron}=[neuron];
    \tikzstyle{output neuron}=[neuron];
    \tikzstyle{hidden neuron}=[neuron];
    \tikzstyle{annot} = [text width=4em, text centered]
    \gen{1}{0}{1}
    \gen{4}{0}{-4}
    \dataset{1}{5.6}{.50}
    \dataset{4}{5.6}{-4.50}
    % \dataset{1}{5.6}{.65}
    % \dataset{4}{5.6}{-4.35}
    \foreach \coord in {1,...,3}
    {
      \draw[fill=black] (0, \coord/2.5-4) circle (.02);
      \draw[fill=black] (-2.1, \coord/2.5-4) circle (.02);
      \draw[fill=black] (4.8, \coord/2.5-4) circle (.02);
    }
    \nn{4}{9}{-1.5}
    \draw[->, semithick] (5.6+1.8,.65-1.25) -- (8.5,-2.5);
    \draw[->, semithick] (5.6+1.8,-4.35-1.25) -- (8.5,-4);
    \tdataset{}{8.8}{2}
    \draw[brace, decoration={raise= .2cm}] (-.7, 1) -- (-1.3, 1);
 %   \draw[brace, decoration={raise= .2cm}] (1.85, 1) -- (1.15, 1);
    \node[align=center] (label1) at (-1.1, 1.5) {Structural gates};
 %   \node[align=center] (label2) at (1.7, 1.5) {Functional gates};
%\draw[brace, decoration={raise= .2cm}] (-1.3, -7.2) -- (-.7, -7.2);
    \draw[brace, decoration={raise= .2cm}] (-.5, -7.4) -- (4.5, -7.4);
    \draw[brace, decoration={raise= .2cm}] (5.5, -7.4) -- (7.6, -7.4);
    \draw[brace, decoration={raise= .2cm}] (8.5, -7.4) -- (14, -7.4);
    \node[align=center] (label3) at (2, -8) {Generators $\hat{f}_1 \dots \hat{f}_4$};
    \node[align=center] (label4) at (6.5, -8) { Generated data};
    \node[align=center] (label5) at (11.3, -8) {Discriminator $T_{\omega}$};

    %\draw[brace, decoration={raise= .2cm}] (#2 + 1.8, #3) -- (#2, #3);
    %\draw[brace, decoration={raise= .2cm}] (#2 + 1.8, #3) -- (#2, #3);
    %\draw[brace, decoration={raise= .2cm}] (#2 + 1.8, #3) -- (#2, #3);

 \end{tikzpicture}
}

